Biased Binary Attribute Classifiers Ignore the Majority Classes

To visualize the regions of interest that classifiers base their decisions on, different Class Activation Mapping (CAM) methods have been developed. However, all of these techniques target categorical classifiers only, though most real-world tasks are binary classification. In this paper, we extend gradient-based CAM techniques to work with binary classifiers and visualize the active regions for binary facial attribute classifiers. When training an unbalanced binary classifier on an imbalanced dataset, it is well-known that the majority class, i.e. the class with many training samples, is mostly predicted much better than minority class with few training instances. In our experiments on the CelebA dataset, we verify these results, when training an unbalanced classifier to extract 40 facial attributes simultaneously. One would expect that the biased classifier has learned to extract features mainly for the majority classes and that the proportional energy of the activations mainly reside in certain specific regions of the image where the attribute is located. However, we find very little regular activation for samples of majority classes, while the active regions for minority classes seem mostly reasonable and overlap with our expectations. These results suggest that biased classifiers mainly rely on bias activation for majority classes. When training a balanced classifier on the imbalanced data by employing attribute-specific class weights, majority and minority classes are classified similarly well and show expected activations for almost all attributes

==> results/error_rates.tex <==
 Attractive          & 0.514 & 0.175     & \bf 0.174 & 0.174 & 0.169 & 0.177 & 0.173 \\
 Mouth Slightly Open & 0.482 & \bf 0.055 & 0.048     & 0.052 & 0.053 & 0.048 & 0.050 \\
 Smiling             & 0.480 & \bf 0.072 & 0.063     & 0.067 & 0.065 & 0.064 & 0.064 \\
 Wearing Lipstick    & 0.470 & \bf 0.065 & 0.037     & 0.052 & 0.054 & 0.043 & 0.049 \\
 High Cheekbones     & 0.452 & \bf 0.126 & 0.102     & 0.113 & 0.132 & 0.104 & 0.118 \\
 Male                & 0.419 & \bf 0.017 & 0.008     & 0.012 & 0.017 & 0.008 & 0.012 \\
 Heavy Makeup        & 0.384 & \bf 0.113 & 0.046     & 0.074 & 0.065 & 0.081 & 0.074 \\
 Wavy Hair           & 0.319 & \bf 0.258 & 0.058     & 0.132 & 0.187 & 0.093 & 0.128 \\
 Oval Face           & 0.283 & \bf 0.598 & 0.077     & 0.255 & 0.286 & 0.319 & 0.308 \\
 Pointy Nose         & 0.276 & \bf 0.629 & 0.055     & 0.209 & 0.336 & 0.209 & 0.243 \\
 Arched Eyebrows     & 0.266 & \bf 0.274 & 0.110     & 0.160 & 0.119 & 0.221 & 0.190 \\
 Big Lips            & 0.241 & \bf 0.651 & 0.076     & 0.264 & 0.353 & 0.269 & 0.297 \\
 Black Hair          & 0.239 & \bf 0.202 & 0.051     & 0.093 & 0.086 & 0.139 & 0.124 \\
 Big Nose            & 0.236 & \bf 0.367 & 0.115     & 0.176 & 0.165 & 0.266 & 0.241 \\
 Young               & 0.779 & 0.055     & \bf 0.300 & 0.116 & 0.137 & 0.151 & 0.140 \\
 Straight Hair       & 0.209 & \bf 0.425 & 0.074     & 0.149 & 0.134 & 0.232 & 0.211 \\
 Bags Under Eyes     & 0.204 & \bf 0.362 & 0.100     & 0.156 & 0.141 & 0.221 & 0.204 \\
 Brown Hair          & 0.204 & \bf 0.248 & 0.074     & 0.107 & 0.115 & 0.205 & 0.188 \\
 Wearing Earrings    & 0.187 & \bf 0.181 & 0.061     & 0.086 & 0.073 & 0.138 & 0.124 \\
 No Beard            & 0.834 & 0.024     & \bf 0.081 & 0.033 & 0.044 & 0.036 & 0.043 \\
 Bangs               & 0.152 & \bf 0.119 & 0.020     & 0.036 & 0.038 & 0.053 & 0.050 \\
 Blond Hair          & 0.149 & \bf 0.153 & 0.017     & 0.035 & 0.048 & 0.067 & 0.065 \\
 Bushy Eyebrows      & 0.144 & \bf 0.326 & 0.031     & 0.073 & 0.147 & 0.110 & 0.116 \\
 Wearing Necklace    & 0.121 & \bf 0.507 & 0.038     & 0.108 & 0.152 & 0.230 & 0.218 \\
 Narrow Eyes         & 0.116 & \bf 0.679 & 0.021     & 0.110 & 0.252 & 0.172 & 0.183 \\
 5 o Clock Shadow    & 0.112 & \bf 0.216 & 0.034     & 0.055 & 0.050 & 0.110 & 0.103 \\
 Receding Hairline   & 0.080 & \bf 0.398 & 0.026     & 0.060 & 0.092 & 0.129 & 0.126 \\
 Wearing Necktie     & 0.073 & \bf 0.159 & 0.014     & 0.025 & 0.036 & 0.060 & 0.058 \\
 Rosy Cheeks         & 0.065 & \bf 0.361 & 0.026     & 0.054 & 0.044 & 0.144 & 0.136 \\
 Eyeglasses          & 0.065 & \bf 0.018 & 0.002     & 0.003 & 0.013 & 0.007 & 0.007 \\
 Goatee              & 0.064 & \bf 0.170 & 0.018     & 0.026 & 0.007 & 0.069 & 0.066 \\
 Chubby              & 0.058 & \bf 0.420 & 0.024     & 0.048 & 0.073 & 0.154 & 0.149 \\
 Sideburns           & 0.056 & \bf 0.116 & 0.019     & 0.024 & 0.014 & 0.070 & 0.067 \\
 Blurry              & 0.051 & \bf 0.476 & 0.010     & 0.029 & 0.061 & 0.110 & 0.108 \\
 Wearing Hat         & 0.049 & \bf 0.078 & 0.004     & 0.007 & 0.028 & 0.015 & 0.016 \\
 Double Chin         & 0.047 & \bf 0.477 & 0.014     & 0.038 & 0.060 & 0.142 & 0.138 \\
 Pale Skin           & 0.043 & \bf 0.491 & 0.007     & 0.028 & 0.048 & 0.147 & 0.142 \\
 Gray Hair           & 0.042 & \bf 0.217 & 0.009     & 0.016 & 0.025 & 0.061 & 0.060 \\
 Mustache            & 0.041 & \bf 0.505 & 0.011     & 0.033 & 0.034 & 0.081 & 0.079 \\
 Bald                & 0.023 & \bf 0.191 & 0.005     & 0.009 & 0.025 & 0.032 & 0.032 \\

